SoccerNet 2023 Challenges Results

The SoccerNet 2023 challenges were the third annual video understanding challenges organized by the SoccerNet team. For this third edition, the challenges were composed of seven vision-based tasks split into three main themes. The first theme, broadcast video understanding, is composed of three high-level tasks related to describing events occurring in the video broadcasts: (1) action spotting, focusing on retrieving all timestamps related to global actions in soccer, (2) ball action spotting, focusing on retrieving all timestamps related to the soccer ball change of state, and (3) dense video captioning, focusing on describing the broadcast with natural language and anchored timestamps. The second theme, field understanding, relates to the single task of (4) camera calibration, focusing on retrieving the intrinsic and extrinsic camera parameters from images. The third and last theme, player understanding, is composed of three low-level tasks related to extracting information about the players: (5) re-identification, focusing on retrieving the same players across multiple views, (6) multiple object tracking, focusing on tracking players and the ball through unedited video streams, and (7) jersey number recognition, focusing on recognizing the jersey number of players from tracklets. Compared to the previous editions of the SoccerNet challenges, tasks (2-3-7) are novel, including new annotations and data, task (4) was enhanced with more data and annotations, and task (6) now focuses on end-to-end approaches. More information on the tasks, challenges, and leaderboards are available on https://www.soccer-net.org. Baselines and development kits can be found on https://github.com/SoccerNet.

==> tables/leaderboard_ball_short.tex <==
\begin{table}[t]
    \caption{Top-3 action spotting leaderboard, complete leaderboard available in Table~\ref{tab:LeaderboardBallSpotting} in the appendix. Main metric for the leaderboard and best performances in bold. Team names with a superscript have provided a summary that may be found in Appendix~\ref{app:ballspotting} or in Section~\ref{sub:ballactionspottingwinner} for the winning team.
    }
    \label{tab:ShortLeaderboardBallSpotting}
    \centering
\resizebox{\columnwidth}{!}{%
    \begin{tabular}{l||c|c|c|c|c||c}
% Title
\multirow{ 2}{*}{Participants} & \multicolumn{5}{c||}{\textbf{mAP}} & \multicolumn{1}{c}{Average-mAP} \\ %\cline{2-7}
&  \textbf{@1} & @2 & @3 & @4 & @5 & tight \\ \midrule
% Teams
\textbf{Ruslan Baikulov} 	&\textbf{86.47} 	&87.98 	&88.28 	&88.18 	&87.95 	&87.91\\
FDL@ZLab 	&83.39 	&85.19 	&85.81 	&86.0 	&86.19 	&85.45\\
BASIK 	&82.06 	&83.39 	&83.86 	&84.04 	&83.91 	&83.57\\
Baseline (PTS)~\cite{Hong2022Spotting}* 	&62.72 	&69.24 	&72.57 	&74.29 	&74.8 	&71.21\\

    \end{tabular}%
}
\end{table}


==> tables/leaderboard_spotting_short.tex <==


\begin{table}[t]
    \caption{Top-3 action spotting leaderboard, complete leaderboard available in Table~\ref{tab:LeaderboardSpotting} in the appendix. Main metric for the leaderboard and best performances in bold. Team names with a superscript have provided a summary that may be found in Appendix~\ref{app:spotting} or in Section~\ref{sub:actionspottingwinner} for the winning team.
    }
    \label{tab:ShortLeaderboardSpotting}
    \centering
\resizebox{\columnwidth}{!}{%
    \begin{tabular}{l||c|c|c||c|c|c}
% Title
\multirow{ 2}{*}{Participants} & \multicolumn{3}{c||}{\textbf{tight Average-mAP}} & \multicolumn{3}{c}{loose Average-mAP} \\ %\cline{2-7}
& \textbf{main} & vis. & inv. & main & vis. & inv. \\ \midrule
% Teams
\bf{SDU\_VSISLAB$^{S1}$} & \bf{71.31} &  76.29  & 54.09 & 78.56  & 81.67 & 69.13 \\
mt\_player$^{S2}$ & 71.10 & 77.22  & 58.5 & 78.79  & 82.02 & 77.62 \\
ASTRA$^{S3}$ &  70.10 & 75.00  & 57.98 & 79.21  & 81.69 &  75.36 \\
Baseline (Yahoo)~\cite{Soares2022Temporally}* & 68.33 & 73.22  & 60.88 & 78.06  & 80.58 & 78.32 \\
    \end{tabular}%
}
\end{table}

